Boosting Order-Preserving and Transferability for Neural Architecture Search: a Joint Architecture Refined Search and Fine-tuning Approach

Supernet is a core component in many recent Neural Architecture Search (NAS) methods. It not only helps embody the search space but also provides a (relative) estimation of the final performance of candidate architectures. Thus, it is critical that the top architectures ranked by a supernet should be consistent with those ranked by true performance, which is known as the order-preserving ability. In this work, we analyze the order-preserving ability on the whole search space (global) and a sub-space of top architectures (local), and empirically show that the local order-preserving for current two-stage NAS methods still need to be improved. To rectify this, we propose a novel concept of Supernet Shifting, a refined search strategy combining architecture searching with supernet fine-tuning. Specifically, apart from evaluating, the training loss is also accumulated in searching and the supernet is updated every iteration. Since superior architectures are sampled more frequently in evolutionary searching, the supernet is encouraged to focus on top architectures, thus improving local order-preserving. Besides, a pre-trained supernet is often un-reusable for one-shot methods. We show that Supernet Shifting can fulfill transferring supernet to a new dataset. Specifically, the last classifier layer will be unset and trained through evolutionary searching. Comprehensive experiments show that our method has better order-preserving ability and can find a dominating architecture. Moreover, the pre-trained supernet can be easily transferred into a new dataset with no loss of performance.

==> sec/0_abstract.tex <==
\begin{abstract}
%Single Path One-Shot Neural Architecture Search is a powerful NAS method due to its simplicity and fast speed. The pipeline consists of a pretraining stage and a search stage. The former trains a supernet based on uniform path sampling and the latter searches architectures and evaluates their performance by loading the supernet weight without fine-tuning.
%However, such performance approximations can be biased and have unsatisfactory fine-grained order-preserving ability.
Supernet is a core component in many recent Neural Architecture Search (NAS) methods especially for one-shot methods, whereby it not only helps embody the search space but also provide a (relative) estimation for the final performance of a candidate architecture. 

Most recent works introduce supernet as relative performance estimators. Thus, order-preserving ability is important for a supernet.
%However, most recent NAS methods have either unsatisfactory global or local order-preserving ability.
We further divide the order preserving ability into global and local order preserving ability, and find that current methods cannot guarantee both at the same time。
This work proposes \textbf{supernet shifting}, a new NAS method. Specifically, after a single-path supernet is trained by uniform sampling, which ensures global order-preserving ability, we introduce a self-adaptive fine-tuning procedure to the evolutionary searching stage.
% First, its fine-grained order-preserving ability is not good enough. Second, it’s difficult to transfer a pretrained supernet to a new dataset, which is also the shortcomings of most of NAS methods.
%In this work, we propose a new search method based on Single Path Supernet. We add a training stage homogeneously with the evolution searching stage. This enables supernet self-adaptively adjust the weight. 
Taking use of the biased sample strategy during evolutionary searching algorithm, the supernet will be shifted to focus on good architecture and forget the noise produced by poor architectures. Thus, our supernet has better local resolution.
Moreover, a pretrained supernet is un-reusable when searching on a new dataset or task, which is also the shortcoming of most one-shot NAS methods. The supernet shifting stage can realize transferring supernet to a new dataset. Specifically, the last classifier layer will be unset and trained through Evolution Searching.
Comprehensive experiments show that our method has better order-preserving ability, and is able to find a dominating architecture on various datasets. Moreover, the pre-trained supernet is reusable and can be easily transferred into a new dataset with no loss of performance.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
\quad 
With the rise of deep learning, experts manually designed powerful and fast neural architectures like VGG~\cite{vgg} and RESNET~\cite{resnet}, which require large amounts of errors and trials.
%With the rise of deep learning, experts are searching for both powerful and fast neural architectures. Usually, the architectures are manually designed like AlexNet and RESNET. Then optimization methods are applied to get the optimal weight.\par
Neural Architecture Search (NAS), an important part of automated machine learning (AutoML), aims to automatically search an optimal architecture in a searching space.

Early NAS approaches~\cite{ref,ref2,ref3,ref4}  adopt a time-consuming pipeline by sampling architectures and training their weights separately.
To speed up the search procedure, many recent approaches introduce performance estimators for each neural architecture. Though there exists a performance estimation gap, the search stage focuses more on the relative ranking of architectures rather than true performance.

Some works~\cite{grasp,snip,naswot} propose zero-cost proxies, which only require one forward step or one backward step. Nevertheless, such zero-cost proxies cannot perform consistently well on diverse tasks~\cite{eznas}. Other works~\cite{ENAS,oneshot} introduce a weight-sharing strategy and build up a supernet that contains all candidate operations and connections in the search space. Once a supernet is trained, all architectures can be quickly evaluated by loading the supernet weight without the time-consuming training procedure. 

Though such a supernet-based performance estimator is widely used in NAS tasks, few works have analyzed its order-preserving ability, i.e. whether the estimated architecture ranking is consistent with true performance ranking. 
In this work, we delve into two aspects of order-preserving ability. 
One is \textbf{global order-preserving ability} to distinguish good architectures from poor architectures. The other is \textbf{local order-preserving ability} to rank top architectures that have good performance.
We argue that both the above abilities are important. Poor global order-preserving abilities will lead to unsatisfactory results since it cannot screen out poor architectures. Poor local order-preserving ability will reduce search efficiency.

%Most recent NAS approaches introduce weight-sharing strategy~\cite{ENAS} and supernet~\cite{oneshot}. Once a supernet is trained, all architectures can be quickly evaluated by loading the supernet weight without the time-consuming training procedure.\par

%Since nearly all NAS approaches retrain the searched architecture from scratch, we only focus on the relative accuracy among different architectures on the searching stage. So we can claim that, the most important feature of the supernet is the order-preserving ability. Specifically, we further divide the order-preserving ability into two aspects,  \textbf{global order-preserving ability} and  \textbf{local order-preserving ability}. 

%to define local and global

%We then theoretically analyze the advantages and drawbacks of current methods on these two aspects.\par

Some NAS approaches, like DARTS~\cite{DARTS} and GDAS~\cite{GDAS}, have good local order-preserving ability but can't ensure global order-preserving ability. They introduce an architecture parameter which is optimized during the supernet training. The architecture parameter leads the supernet focus on part of the architectures, thus improving local discernment. However, some previous works~\cite{SPOS}~\cite{drop}~\cite{partial} have pointed out that the parameters are deeply coupled and the architecture parameter may introduce an early bias. The search direction may be led wrongly in the early stage and therefore global order-preserving ability can't be guaranteed.

Other works like SPOS~\cite{SPOS} and FairNAS~\cite{FAIR} ensure global order-preserving ability. They remove the architecture parameter and treat NAS as a two-stage process. First, a single-path supernet is trained by uniform sampling and all architectures' weights are optimized simultaneously. Then, an evolutionary algorithm is used to search for optimal architecture. This method ensures fairness by uniform sampling so the global order-preserving ability is better.
However, such methods can not guarantee local order-preserving ability. We select the top-10 architectures during the search stage and retrain them separately. The top-10 results are similar in chosen-blocks. The \emph{Kendall's tau rate} of the accuracy in supernet and after retrain is only 0.17. This shows that the local prediction is unreliable. The problem is that since weight-sharing strategy is used, the weights of different architectures are not fully decoupled. Some previous works ~\cite{m1,m2,m3,m4,m5} point out that the gradient direction of different architectures may conflict in the weight-sharing strategy. Uniform sampling strategy avoids early bias and ensures the overall fairness of comparisons, but it's not precise enough in local comparison since other architectures may produce noise. In fact, we want our supernet to focus on some local superior architectures. Inferior architectures may produce noise and thus should be neglected.

In this work, we propose to adopt the advantages and avoid the shortcomings of the two previous manners to ensure both global and local order-preserving ability.
However, such a method is not straightforward. Uniform sampling strategy isn't precise enough to improve local order-preserving ability. Biased sampling strategy is needed to focus on some local superior architectures and increase local discernment, but it can lead to improper bias and hurt global order-preserving ability.
%These two goals seem to conflict with each other. 
To this end, we propose a new NAS pipeline ensuring both global and local order-preserving ability.
To ensure global order-preserving ability, We first train a superent by uniform sampling to avoid early bias and ensure the overall fairness. To improve local order-preserving ability, we add a \textbf{supernet shifting} stage during the evolutionary search stage. Specifically, We finetune the supernet by tens of iterations before evaluation when an architecture is sampled. Since the evolutionary algorithm tends to sample superior architectures, we gradually shift the supernet to focus on superior architectures and forget the inferior ones. Thus, for the superior architectures, our shifted supernet has better local discernment and better local order-preserving ability. For inferior architectures, accuracy remains or decreases, and this doesn't matter since they should be eliminated during the search process. By experiment, our method can find a dominating architecture with a small additional time cost.

Moreover, our method has better transferability compared to other one-shot NAS methods that require to train a new supernet for a new dataset. In contrast, our method can directly adopt the original supernet and fine-tune the weight during the search procedure. Plenty of previous work on transfer learning and the success of large pre-trained models~\cite{bert,MAE} proves that the weights can be inherited and only need some small changes for different tasks. This provides a theoretical basis for us to transfer supernet to different datasets.

Overall, our contributions can be summarized as follows:

%Moreover, most NAS methods have poor transferring ability, especially one-shot NAS method. For a new dataset, we need to train a new supernet. This is time-consuming and has high requirements on hardware, which strongly limits the wide application of NAS approaches.\par

%In fact, plenty of works on transfer learning and the success of large pre-trained models prove that the weights can be inherited and only need some small changes for different tasks. This provides a theoretical basis for us to transfer supernet to different datasets.\par

%Our method can flexibly transfer a supernet to a new dataset. Specifically, we keep most part of supernet and only reset the last fully-connected classifier layer. Then during evolutionary searching stage, since we finetune the supernet when sampling an architecture, the supernet fits the new dataset quickly after only several architectures are sampled. Therefore, the supernet can be reused with no loss of performance.\par

%In this work, we propose supernet shifting, a simple but effective method. Our contributions can be summarized as follows:

\textbf{1) Comprehensive analysis about order-preserving ability for NAS methods.}
Many NAS methods adopt proxies to estimate performance to speed up the search process, making order-preserving ability a general metric. In this work, we further define global and local order-perserving ability and verify the dilemma of current NAS method. 

\textbf{2) A stable strategy improving both global and local order-preserving ability.}
%Comprehensive comparison experiments on various datasets have shown the general effectiveness of our approach. Our method improves both global and local order-preserving ability, and thus can obtain a better architecture on different datasets with little additional time cost. \par
This work introduces supernet shifting, a simple but effective NAS method to improve global and local order-preserving ability. Specifically, we self-adaptively revise the supernet during the evolutionary search process. Due to the exploitation property of EA, weights of good architectures can be gradually fine-tuned and poor architectures are gradually eliminated. Compared with previous method, ours is more precise and more in line with the essential requirements of NAS than paying equal attention to every architecture, and is more stable than introducing early bias.
%Our strategy is more closed to the essence of NAS than ensuring strict fairness, and is more robust than introducing early bias.


\textbf{3) A flexible and efficient strategy realizing transferring during searching.}
 %Our method can reuse the pre-trained supernet on different downstream tasks. By experiment, our method accelerate the searching stage by tens of times and can even find a dominating architecture in comparison with training a new supernet. To the best of our knowledge, this is the first time a supernet can be transferred to different downstream datasets.\par
 Our method neatly realize the transfer of supernet by reusing the feature encoder part of pre-trained supernet. The simplicity allows flexible design of decoders to better fit different tasks and datasets. And gradual transferring with searching further ensures time efficiency. To the best of our knowledge, this is the first time an entire supernet can be transferred.
 
\textbf{4) Strong Performance.}
Comprehensive experiments on various datasets in Sec.~\ref{4} have shown the general effectiveness of our method. It improves both global and local order-preserving ability. The kendall's coefficiency largely raises from 0.1 to 0.7. Therefore, it can obtain a dominating architecture on different datasets. The Flops can be reduced by $5M$ and the accuracy increases by $0.3\%$ on ImageNet-1K. Besides, it is also less sensitive on the supernet training stage. For transferability, it can largely accelerate searching process for ten times compared with SPOS without performance loss.


%-------------------------------------------------------------------------


==> sec/2_formatting.tex <==
\section{Related Works}
\label{sec:formatting}

%-------------------------------------------------------------------------
\subsection{One-Shot NAS}
 Early NAS approaches~\cite{ref,ref2,ref3,ref4} adopt a straightforward but time-consuming pipeline. Different architectures are sampled and their weights are usually trained from scratch separately to evaluate the performance. The time cost is usually unaffordable due to the difficulty of training a neural network.

\emph{ENAS} ~\cite{ENAS} introduces weight-sharing strategy so that different architectures can be jointly optimized. This greatly speeds up the NAS process and makes searching on large-scale datasets feasible.

Based on weight-sharing strategy, \emph{One-Shot NAS}~\cite{oneshot} further adopts path dropout technique to train a supernet. Once a supernet is trained, the architectures can simply inherit weight from it and this enables fast evaluation. Most follow-up works adopt this strategy. They can be divided into two classes roughly based on their searching space.

Some works ~\cite{DARTS,GDAS,pdarts,proxy,dense} use contiguous relaxation and adopt contiguous searching space. They introduce a learned architecture parameter. Thus, gradient decent method can be used to optimize the supernet weight and the architecture parameter.

Another line of works ~\cite{SPOS,FAIR,single} adopt discrete searching space and apply sampling algorithm. They treat NAS as a two-stage problem. In supernet training stage, only one path is sampled and optimized from the searching space. Then different searching algorithms like evolutionary search can be applied to find the optimal architecture, which is usually more stable and easier to optimize.

A widely used NAS method \emph{SPOS}~\cite{SPOS} falls into the second category. \emph{SPOS} trains a supernet by uniform sampling and applies evolutionary searching algorithm to search for optimal architecture. This is our main baseline.


\subsection{EA-based NAS}
\quad Evolutionary algorithm is widely used in multi-object optimizing problem. It simulates the process of biological evolution process. New candidates are created by crossover and mutation.

\emph{Large-Scale Evolution of Image Classifiers} ~\cite{ea1} first introduces evolutionary algorithm into NAS problem. New candidate architectures are produced and trained separately. Many later works ~\cite{hie,gen} adopt evolutionary algorithm, but the searching cost is unaffordable due to the high training cost.

After the proposal of weight sharing strategy and supernet, evolutionary algorithm is widely used in the works ~\cite{SPOS,FAIR} using discrete searching space as a sample strategy during searching stage. Specifically, \emph{SPOS}~\cite{SPOS} apply evolutionary searching algorithm first on a single-path supernet while \emph{FairNAS}~\cite{FAIR} uses NSGA-\uppercase\expandafter{\romannumeral2}, a slightly revisited evolutionary searching algorithm. It's widely accepted that evolutionary searching algorithm is more efficient than random searching since it takes use of the current evaluation results.

\subsection{Transferability in NAS}
\quad Transfer learning aims to find an effective way to transfer the knowledge learned from a source domain to a target domain. The definition of knowledge and domain can be varied. Usually, the parameters of the pre-trained model are carefully fine-tuned and the structure is often adjusted to adapt it to the target domain.

Transferability is an important feature for NAS method, since it can significantly reduce the time cost and hardware restriction for NAS application. However, few NAS methods find an effective way to realize tranferability. Some NAS methods~\cite{DARTS,SNAS} are time-consuming, so they first search on a small-scale dataset like Cifar10, then extend the searched architecture to large-scale datasets like ImageNet-1K directly. This transfer mode could be unreliable because of the diverse data distribution. Some recent works ~\cite{trans} introduce meta learning to achieve transferability. However, this is often complicated. The model and hyperparameters have to be carefully designed and it usually lacks explainability.

To the best of our knowledge, no previous work has transferred an entire pre-trained supernet to a new dataset. 

%-------------------------------------------------------------------------


==> sec/3_method.tex <==

\section{Method}
\begin{table*}[tb!]
  \centering
  
  \begin{tabularx}{\textwidth}{|>
  {\centering\arraybackslash}m{1.9cm}<{\centering}|>{\centering\arraybackslash}m{2.4cm}<{\centering}|>{\centering\arraybackslash}m{1.6cm}<{\centering}|>{\centering\arraybackslash}X<{\centering}|>{\centering\arraybackslash}m{1.5cm}<{\centering}|>
  {\centering\arraybackslash}m{1.5cm}<{\centering}|>
  {\centering\arraybackslash}m{1.7cm}<{\centering}|}
    \hline
     \textbf{Method} & \textbf{Supernet training} & \textbf{Searching} & \textbf{Attention on different architectures} & 
     \textbf{global resolution} &
    \textbf{local resolution}&
    \textbf{transferable supernet}\\
    \hline
    DARTS~\cite{DARTS} & gradient descent, path dropout & / & biased by architecture parameter at start  &\times &\checkmark & \times \\
    \hline
    One-Shot~\cite{oneshot} & path dropout & random search & equal attention  &\checkmark &\times &\times \\ 
    \hline
    SPOS~\cite{SPOS} & uniform sampling & EA & equal attention &\checkmark &\times  &\times \\
    \hline
    FairNAS~\cite{FAIR} & strict fairness sampling & EA &
    strictly equal attention&\checkmark & \times & \times \\
    \hline
    Ours & uniform sampling & EA with shifting &biased by validation after uniform training & \checkmark &\checkmark &\checkmark\\
    \hline
  \end{tabularx}
  \caption{An overview and comparison of different one-shot NAS methods. By adding supernet shifting, our method introduce extra attention on partial architectures based on its validation performance. Therefore, the local resolution can be improved and the training process is stable. Besides, ours has the best transferrability.}
  \label{overview}
\end{table*}
\subsection{Revisiting from order-preserving perspective}
To have a deeper understanding of different NAS methods and their advantages as well as shortcomings, we use some mathematical expressions to show their training pipelines and training goals. Thus, we need to make some definitions for the following mathematical expressions.

In the following expressions, $\theta$ represents learned architecture variable, $\alpha$ represents different architectures,  $\tau(\alpha)$ represents a sampling distribution of architecture $\alpha$ and $\mathcal{A}$ represents a uniform sampling distribution of all architectures. $\mathcal{W_{\mathcal{A}}}$ represents the weight of supernet. and $\mathcal{W}_{\alpha}$ represents the weight of architecture $\alpha$ inherited from the supernet.

As discussed above, we divide the previous one-shot NAS into two main ways. Some~\cite{DARTS,GDAS,pdarts,proxy,dense} use continuous search space and introduce a learnable architecture variable $\theta$. Their optimization steps are
\begin{equation}
  (\theta, \mathcal{W}_{\theta}) = \mathop{\arg\min}\limits_{\theta, \mathcal{W}}\mathcal{L}_{train}(\mathcal{N}(\mathcal{A}(\theta),\mathcal{W}))
  \label{eq:4}
\end{equation}

The existing of $\theta$ leads the supernet to focus on a local set of architectures, and this improves the local resolution near $\theta$. This kind of method theoretically works well if $\theta$ is optimal. But $\theta$ is learned together with $\mathcal{W}_{\theta}$ and this may introduce early bias. So the jointly learning mode may get a totally wrong $\theta$, the supernet may be misled and trapped into a local optimal architecture, which hurts global order-preserving ability.

Many other works~\cite{SPOS,FAIR,single} use discrete search space and get rid of the architecture variable $\theta$. They first train a supernet by uniform sampling and apply searching algorithms to find the optimal architecture based on their performance on the supernet. Their optimization steps are sequential, which can be illustrated as
\begin{equation}
  \mathcal{W_{\mathcal{A}}} = \mathop{\arg\min}\limits_{\mathcal{W}}\mathcal{L}_{train}(\mathcal{N}(\mathcal{A},\mathcal{W}))
  \label{eq:5}
\end{equation}
\begin{equation}
  \alpha^{*} = \mathop{\arg\max}\limits_{\alpha}ACC_{val}(\mathcal{N}(\alpha,\mathcal{W}_{\alpha}))
  \label{eq:51}
\end{equation}

By removing $\theta$ and applying uniform sampling, it ensures the fairness of comparison and the global order-preserving ability. However, it isn't precise enough for local comparison because it pays equal attention to every single architecture. \par
Our work aims to achieve both global and local order-preserving ability. Section \ref{3.2} aims to ensure the former and Section \ref{3.3} aims to improve the latter.\par

\subsection{Single-Path Supernet Training}
\label{3.2}
\quad First, we construct a single-path supernet. The construction and the training process of supernet follow SPOS~\cite{SPOS}. The supernet has a series of choice blocks, and each choice block has several choices. Only one choice is invoked at the same time. The supernet is trained by uniform sampling. For each iteration, we uniformly sample an architecture and optimize the corresponding weight. The optimization process can be defined as:
\begin{equation}
  \mathcal{W_{\mathcal{A}}} = \mathop{\arg\min}\limits_{\mathcal{W}}\mathcal{L}_{train}(\mathcal{N}(\mathcal{A},\mathcal{W}))
  \label{eq:6}
\end{equation}

Experiments on Section \ref{4.3} prove that global order-preserving ability is good enough for the supernet trained by uniform sampling and it won't decay after our supernet shifting stage. However, the local order-preserving ability needs to be further improved.

\subsection{Supernet Shifting}
\label{3.3}
After training a supernet by uniform sampling, the variance of different architectures' accuracy is relatively small. This is enough for global comparison. The supernet can distinguish between good architecture and poor architecture. However, it's not capable enough to distinguish the best architecture from several similar architectures, and this seriously affects its performance. To solve the problem, we need a new sampling strategy which can lead the supernet to lay more emphasis on superior architectures.\par
The supernet weight should be shifted based on the current performance of different architectures. Specifically, the architectures which performs better should be more emphasized. Thus, these architectures should be sampled more frequently. The process can be depicted as:
\begin{equation}
  \mathcal{W^{*}_{\mathcal{A}}} = \mathop{\arg\min}\limits_{\mathcal{W}}\mathbb{E}_{\alpha \sim\tau(\mathcal{\alpha})}[\mathcal{L}_{train}(\mathcal{N}(\alpha,\mathcal{W}_{\alpha}))]
  \label{eq:7}
\end{equation}

The prior distribution of $\tau(\alpha)$ is important. If $\tau(\alpha)$ is a uniform distribution, this equation is the same as Eq.\eqref{eq:6}. As discussed above, for architecture $\alpha$, we want the sampling probability $\tau(\alpha)$ and the performance of $\alpha$ to be positively correlated, i.e.
\begin{equation}
r[\tau({\alpha}),ACC_{val}(\mathcal{N}(\alpha,\mathcal{W_{\alpha}}))]\ > \ 0
  \label{eq:71}
\end{equation}

Thus, after the shifting stage, the supernet is led to focus on better architectures. We then search for the optimal architecture based on the shifted supernet.
\begin{equation}
  \alpha^{*} = \mathop{\arg\max}\limits_{\mathcal{\alpha}}ACC_{val}(\mathcal{N}(\alpha,\mathcal{W^{*}_{\alpha}}))
  \label{eq:8}
\end{equation}

Compared with those biased architecture sampling strategy using architecture parameter $\theta$, our sampling strategy is obviously more precise and more reliable since the supernet training stage\ref{3.2} ensures overall fairness and the sampling distribution is determined by their evaluation performance directly.

Only one problem remains to be solved. Finding a proper sampling distribution according to Eq.\eqref{eq:71} isn't an easy thing.

We take use of the property of evolutionary searching algorithm to solve the problem. Evolutionary searching algorithm is often used in discrete searching space. It's an effective method for solving multi-objective optimization problems. The main difference between evolutionary searching algorithm and random sampling is that, for different architectures, the probability of being sampled by evolutionary searching algorithm is different. The evolutionary searcher tends to sample the architectures which are similar to  the current superior architectures. So better architectures are sampled more frequently in evolutionary searching. Therefore, we can claim that the sampling probability of evolutionary searching algorithm satisfies Eq.\eqref{eq:71}
\begin{figure}[t]
  \centering
   \includegraphics[width=\linewidth]{sec/img/supernet-shifting.png}
   \caption{The trajectory of our Supernet Shifting process. We sample 5 superior architectures according to searching result and 5 random architectures. We monitor their accuracy on different iterations of evolutionary searching. The iteration 0 represents the original supernet trained by uniform sampling. We can see that the shifting supernet gradually focus on superior architectures while forget inferior ones, and the coarse-grained resolution increases.}
   \label{shifting}
\end{figure}

Thus, we implement Eq.~\ref{eq:7} and Eq.~\ref{eq:8} homogeneously and realize supernet shifting together with evolutionary searching. Specifically, when an architecture is sampled in evolutionary searching stage, we first fine-tune the supernet with a small learning rate for tens of iterations. Then, we evaluate the accuracy of this architecture based on the fine-tuned supernet. Thus, supernet will focus more on this particular architecture and its local similar architectures. After sufficient architectures are sampled, the supernet will be shifted to foucs on a local set of good architectures due to the biased sampling distribution. This improves the precision for local comparison.

Fig.~\ref{shifting} shows the supernet shifting process during evolutionary searching stage. The accuracy increases for superior architectures while remains or even decreases for inferior ones. This verifies our assumption.

Since supernet keeps shifting in searching, we have to eliminate the bias produced by the changing supernet. Therefore, repeatedly sampling should be allowed. Specifically, for a single particular architecture, we allow a new sample in each iteration of evolutionary algorithm and we will update its latest accuracy. After each iteration, we keep the top-50 different architectures for later mutation and crossover process.

In experiment at Sec.~\ref{4.2} and Sec.~\ref{4.3}, adding the additional shifting stage improves the local order-preserving ability on the superior architectures searched by evolutionary searching algorithm, and the overall performance of supernet on various architectures decreases, especially for those poor architectures. This confirms that the shifting stage leads the supernet focus on superior architectures while forgetting others. And we get dominating architectures on different datasets by applying supernet shifting.

Since we implement supernet shifting and architecture searching homogeneously, and the shifting process need few iterations for training comparing with evaluation, the additional time cost is quite little. Take ImageNet-1K as an example, the total time for evolutionary searching stage only rises from 15 GPU hours to 17 GPU hours.

\subsection{Supernet Transferring}
\quad The lack of transferring ability is a common problem for previous NAS methods. For a new dataset, most of the previous methods need to train a new supernet before searching stage. This is quite time-consuming, which may need several GPU days.

The success of transfer learning and pre-trained models has shown the inner-correlation of different downstream tasks and different datasets. Our method is inspired by fine-tuning, which is one of the most straight-forward and effective implementations of transfer learning.

To transfer the pre-trained supernet to a new dataset, we keep the feature-extraction part of the supernet and only set a new  fully-connected layer for prediction. The supernet is also fine-tuned for tens of iterations when an architecture is sampled in the evolutionary searching algorithm. Since the feature extraction part has a strong internal correlation on different datasets, only prediction layer needs to train from scratch. So the supernet is quickly shifted to a new dataset after several architectures are sampled. The searching algorithm can work properly.

We also try a different mode, freezing the feature extraction part of supernet and only fine-tuning the final prediction layer. In experiment, fine-tuning the whole supernet works better, especially on CIFAR-100 dataset. This is probably because ImageNet-1K dataset isn't large-scale enough. Thus, the general knowledge learned can't eliminate the noised produced by the gap of data distribution. Moreover, since we adopt a lightweight search space, fine-tuning the whole supernet isn't time-consuming. If a more complicated supernet is pre-trained on a larger-scale dataset, the second mode may be better.

Note that the size of images may vary in different datasets, we try two different solutions. The first solution is to simply resize the image into a fixed size like $224\times224$, while the second solution is to set an up-sampling or down-sampling layer in the network. This layer is also initialized and trained during the evolutionary searching algorithm like the prediction layer. By experiment, the former simpler method works better.

In the experiment, we find the transferring supernet converges quickly after sampling several architecture. And after 4 epochs of evolutionary searching, the transferring supernet achieves nearly the same accuracy as a new supernet which is trained for 80 thousand iterations on the new dataset. This strongly confirms that the supernet is theoretically transferable.

Note that our transferring method is time-saving with no loss of performance. Since no new supernet is trained, we make the searching process 9 times faster and even get a dominating architecture comparing with training a new supernet on Imagenet-100 dataset.

\subsection{Summary and Remarks}
\quad We propose a new pipeline of NAS problem. Comparing to the two previous pipelines, our method combines the advantages while overcoming the disadvantages. Introducing supernet shifting both ensures global and local order-preserving ability.

First, training a single-path supernet with uniform sampling ensures the fairness. Then, based on the performance of the architectures instead of a learned architecture parameter, we realize a self-adaptive architecture sampling strategy and thus the supernet can be shifted to focus on superior architectures and forget the others during searching. This gradually removes the noise created by inferior architectures and increases the local resolving ability. And this similar process can be used to transfer a pre-trained supernet to a new dataset.

Our method also inherits the flexibility and simplicity of two-stage NAS. Multiple constraints can be added in the evolutionary searching stage to restrict the maximum Flops, parameters and latency. Therefore, it can be conveniently applied to various occasions in real life.



==> sec/4_experiment.tex <==
\section{Expermient}
\label{4}
\subsection{Experiment Setting}
\textbf{Dataset.}  To show the general effect of our method, three different datasets are used. The biggest dataset is \emph{Imagenet-1K}~\cite{image}, which contains 1000 different classes, over one million images for training and 50000 images for validation. \emph{Imagenet-1K} is the most important dataset in our experiment. 
Since getting retrain performance of a large number of architectures on \emph{Imagenet-1K} is time-consuming, we also use \emph{Imagenet-100} dataset. \emph{Imagenet-100} is a dataset sampled from \emph{Imagenet-1K}. It contains 100 classes and each class contains 1300 images for training and 50 images for validation. \emph{Imagenet-100} dataset is mainly used to evaluate the order-preserving ability and the performance of supernet transferring.
Besides, we also use Cifar-100~\cite{cifar} in supplementary experiments.


\textbf{Searching Space.}Our searching space also follows our main baseline SPOS. It is based on ShuffleNet-V2~\cite{shuffle}, which is a powerful lightweight network. Table~\ref{supernet.} shows the architecture of our supernet. There are total 20 searching blocks and 4 choices for each block. The total searching space is $4^{20}$. We use $FLOPS\leq330M$ as complexity constraint in evolutionary searching as well.


\textbf{Training.}  For the training of supernet and the retraining of the searched architectures, we use the same setting (including hyper-parameters, data-augmentation strategy, learning-rate decay, etc.) as SPOS. The batchsize is 1024, the supernet is trained for 150000 iterations and the searched architecture is trained for 300000 iterations on ImageNet-1K. For ImageNet-100, the batchsize is 256, the supernet is trained for 80000 iterations and the searched architecture is trained for 120000 iterations. To further ensure fairness, we use the same supernet weight for different searching algorithms if the searching space is the same.

\begin{table}[tb!]
  \centering
  \begin{tabular}{|c|c|c|c|c|}
    \hline
    \textbf{Input size} & \textbf{Blocks} & \textbf{Channels} & \textbf{Repeat} & \textbf{Stride} \\
    \hline
    $224^{2}\times3$ & $3\times3$ conv &16 & 1 & 2\\
    $112^{2}\times16$ & CB & 64 & 4 & 2 \\
    $56^{2}\times64$ & CB & 160 & 4 & 2 \\
    $28^{2}\times160$ & CB & 320 & 8 & 2 \\
    $14^{2}\times320$ & CB & 640 & 4 & 2 \\
    $7^{2}\times640$ & $1\times1$conv & 1024 & 1 & 1 \\
    $7^{2}\times1024$ & GAP & 1024 & 1 & - \\
    1024 & fc & 1000 & 1 & - \\
    \hline
  \end{tabular}\vspace{-5pt}
  \caption{The design of our Supernet. CB means choice block. GAP means global average pooling. Stride means the stride of the first layer in each block}
  \label{supernet.}
\end{table}

\subsection{Searching Result}
\label{4.2}
 For comparison, we try multiple searching algorithms and retrain the searched architecture respectively. It involves:
 
1) random select five architectures and choose the best architecture according to retrain performance

2) train a supernet by uniform sampling and use random search to select the best architecture from 100 candidates according to supernet evaluation

3) SPOS (train a supernet by uniform sampling and apply evolutionary searching algorithm.)

4) FairNAS (train a supernet with strict-fairness sampling and apply evolutionary searching algorithm.)

Table~\ref{result} shows retrain result on ImageNet-1K of different methods. We get a dominating architecture which has the lowest flops and the highest accuracy.

\begin{table}[tb!]
  \centering
  \begin{tabular}{|c|c|c|c|}
    \hline
    \textbf{Architectures} & \textbf{Flops} & \textbf{Top-1 acc} & \textbf{Top-5 acc}\\
    \hline
    Random select & 324M & 73.29 & 91.01 \\
    Supernet + random  & 326M & 73.52 & 91.44 \\
    SPOS(channel) & 323M & 74.01(74.30) & 92.25 \\
    FairNAS & todo & todo & todo \\
    Ours & \textbf{318M} & \textbf{74.28} & \textbf{92.92} \\
    \hline
  \end{tabular}\vspace{-5pt}
  \caption{The retrain result on Imagenet-1K of different searched architectures. Our method refers to supernet training + supernet shifting + NSGA. Some top-1 acc is reported as the form of x(y). x shows the result retrained by us and y shows the result proposed on their works. To ensure fairness, for SPOS and FairNAS, we only adopt its training pipeline. The search space is all based on ShuffleNet-V2.}
  \label{result}
\end{table}
\begin{table}[tb!]
  \centering
  \begin{tabular}{|c|c|c|}
    \hline
    \textbf{Method} & \textbf{Flops} & \textbf{Top-1 acc} \\
    \hline
    Random select & 312M & 85.42  \\
    Supernet + random  & 304M & 85.41 \\
    SPOS(channel) & 304M & 85.50 \\
    FairNAS & 300M & 85.44 \\
    Ours & \textbf{299M} & \textbf{85.61} \\
    \hline
  \end{tabular}\vspace{-5pt}
  \caption{The retrain result on ImageNet-100 dataset. All the settings are the same as table .\ref{result}}
  \label{result100}
\end{table}
We also conduct the comparison experiment on ImageNet-100 dataset. The result is shown in Table~\ref{result100}. Our method also finds a dominating architecture. This proves the general effect of our method. 

The scaling performance is an important feature. Thus, we use different depth multipliers to test the scaling performance. Depth multiplier is a simple but effective hyperparameter. By scaling the number of channels, it scales the parameters and flops for architecture. Thus, architectures are expected to be able to flexibly fit different hardware restrictions.

By comparing with SPOS in Fig.~\ref{scale}, our method outperforms SPOS under every depth multiplier. This proves the scalability of our searching method.
\begin{figure}[t!]
  \centering
   \includegraphics[width=0.95\linewidth]{sec/img/scale.png}
\vspace{-5pt}
   \caption{We choose 5 depth multipliers: 0.5, 1.0, 1.5, 2.0 and 4.0. For each we train a new supernet to which we apply our method and the SPOS method. Then, we retrain the searched architecture separately and compare the results on ImageNet-100.}
   \label{scale}
\end{figure}


\subsection{Order-preserving Ability}
\label{4.3}

As discussed before, for one-shot NAS problem using supernet as relative performance predictor, the most or even the only important feature of supernet is the order-preserving ability between supernet performance and retrain performance. Since it's time-consuming to get the retrain accuracy of a large number of architectures, we use ImageNet-100 in this experiment.

We analyze the global order-preserving ability and the local order-preserving ability separately. Specifically, We choose 10 searched architectures as good architectures and 20 random architectures as poor architectures. Each architecture is retrained from scratch for 50000 iterations. We have verified that all 10 good architectures are better than the 20 poor architectures after retraining. Global order-preserving ability means whether the model is able to distinguish good architectures and poor architectures, so we counted how many of the top-10 architectures evaluated by supernet in the overall 30 architectures are the ten good architectures. Ideally, this should be $10$. And local order-preserving ability refers to whether the supernet can predict the relative performance of similar good architectures. So we introduce Kendall's tau coefficient as metric. Kendall's tau coefficient is an important feature indicating the positive correlation of two ranks. We evaluate Kendall's tau coefficient of the 10 good architectures to evaluate the prediction by supernet of relative performance. Ideally, this should be $1$.

\begin{figure}[t!]
  \centering
   \includegraphics[width=\linewidth]{sec/img/order.png}
\vspace{-5pt}
   \caption{Experiments on global and local order-preserving ability. Number of good architectures predicted correctly as the top-10 architectures indicates the global ranking. The Kendall's tau coefficient of the 10 good architectures indicates the local consistency.}
   \label{order}
\end{figure}
Fig.~\ref{order} shows the result of our experiment. We can see that for the supernet trained by uniform sampling strategy, the global ranking is quite ideal but the local consistency still needs to be improved. At the beginning of the searching stage, both the global ranking and the local consistency decreases. This is probably because the searching experience is not enough for evolutionary searching algorithm and thus the sampling doesn't satisfy Eq.~\ref{eq:71}. After several iterations of evolutionary algorithm, we can see a contiguous improving of local consistency and global ranking. This verifies that by using a reliable biased sample strategy like ours, the local order-preserving ability can be improved. After 15 iterations, the local Kendall's tau rate achieves a high score and remains nearly unchanged, which indicates the converge, and ensures the fairness of final comparison.

We can see a gap between the converging result and the ideal case. We've tried extending the evolutionary searching algorithm and carefully selecting proper hyperparameters, but the gap still remains. We think this is the limit of weight sharing strategy and is quite hard to overcome.

\subsection{Supernet Transfer}
 To evaluate the transferability of our method, we first train a supernet on ImageNet-1K and use our method to transfer the supernet to Imagenet-100 and Cifar100 to search for the optimal architecture. We set three different method for comparison.

1. choose the architecture searched on ImageNet-1K and directly transfer it to downstream dataset.

2. train a new supernet on downstream dataset by uniform sampling then apply evolutionary searching algorithm.

3. train a new supernet on downstream dataset by uniform sampling and add supernet shifting stage during evolutionary searching algorithm.

Table~\ref{resulttransfer} and Table~\ref{CIFARtransfer} show the result of our experiments. Our transferring method can reuse the supernet and speed up the search process for a new dataset significantly. Meanwhile, the search quality doesn't decrease. Instead, we even find dominating architecture in ImageNet-100. This shows the supernet which is pre-trained on large-scale datasets like ImageNet-1K contains general knowledge and can improve performance on downstream datasets.

Specifically, the relative transferring performance on ImageNet-100 is better than Cifar-100. This makes sense theoretically since the data distribution on ImageNet-100 is much closer to ImageNet-1K, on which the supernet is trained. And we find our transferring method usually prefers architectures with lower flops and fewer parameters. This is probably because simpler architectures usually converge faster and thus they can occupy an advantageous position at the start of evolutionary searching.

\begin{table}[tb!]
  \centering
  \begin{tabular}{|c|c|c|c|}
    \hline
    \textbf{Method} & \textbf{Flops} & \textbf{Top-1 acc} & \textbf{Time cost} \\
    \hline
    origin architecture & 307M & 85.50 & / \\
    new supernet & 304M & 85.50 & 48\\
    new supernet + shifting  & \textbf{299M} & 85.61 & 50\\
    Ours & 299M & \textbf{85.83} & 6 \\
    \hline
  \end{tabular}
  \caption{The retrain result on different transferring methods on ImageNet-100. Time cost consists of training a supernet and applying a searching algorithm and is measured in GPU hours.}
  \label{resulttransfer}
\end{table}
\begin{table}[tb!]
  \centering
  \begin{tabular}{|c|c|c|c|}
    \hline
    \textbf{Method} & \textbf{Flops} & \textbf{Top-1 acc} & \textbf{Time cost} \\
    \hline
    origin architecture & 233M & 74.73 & / \\
    new supernet & 228M & 75.40 & 20\\
    new supernet + shifting & 230M & \textbf{75.62} & 21\\
    Ours & \textbf{226M} & 75.38 & 3 \\
    \hline
  \end{tabular}
  \caption{The retrain result on different transferring methods on CIFAR-100. Time cost is all measured in GPU hours.}
  \label{CIFARtransfer}
\end{table}

\subsection{Time Cost Analysis}
 Since our method involves our supernet shifting stage together with evolutionary searching stage, the additional time cost is rather small. Moreover, we fine-tune the supernet during supernet shifting stage, this actually lowers the requirements of supernet. Compared with SPOS~\cite{SPOS}, We only need a rough global prediction on different architectures, and the local prediction can be learned and improved during the supernet shifting stage. Thus, the supernet training iterations can be shortened and the performance won't be largely affected.

In experiment shown in Table~\ref{time}, we shorten supernet the training stage from 150K iterations to 100K iterations. Under the same flops, the top-1 accuracy searched by our method only lowers by 0.1, while the accuracy searched by SPOS lowers by 0.4.

Therefore, under some resource-limited situations where the supernet cannot be trained for sufficient iterations and thus can't provide accurate estimation, our method can help to maintain performance.
\begin{table}[tb!]
  \centering
  \label{time}
  \begin{tabular}{|c|c|c|c|}
    \hline
    \textbf{Method} & \textbf{Training} & \textbf{Search} & \textbf{Top-1 acc} \\
    \hline
    SPOS & 150 & 17 & 73.91 \\
    ours & 150 & 20 & 74.11\\
    SPOS(short training) & 100  &17 & 73.52\\
    ours(short training) & 100 & 20 & 73.96 \\
    \hline
  \end{tabular}
  \caption{Time cost of different methods on ImageNet-1K dataset. Specifically, the total searching time is divided into supernet training time and evolutionary searching time. The time cost is all measured in GPU hours and the top-1 accuracy is all estimated under the same Flops.}
  \label{time}
\end{table}
\label{tab:time_cost}

==> sec/5_conclusion.tex <==
\section{Conclusion and Outlook}
\quad In this work, we have proposed supernet shifting, a strong and flexible method for xxx. With little additional time cost, the supernet can focus on superior architectures by utilizing a reliable sampling strategy. Thus, both local and global order-preserving ability can be ensured. Besides, we can transfer the supernet to a new dataset in a simple way. This gives space for developing new NAS pipelines for future study. Most current NAS methods tend to define a small-scale proxy dataset from a large-scale dataset and search for the optimal architecture on the proxy dataset. This is often tricky and time-consuming. We believe a supernet pre-trained on a large-scale dataset will be open source and can be transferred to other datasets effectively. Thus, no time-consuming supernet training is needed and we can get an optimal architecture by only applying searching algorithm on the pre-trained supernet for different datasets. This will significantly reduce the time cost, hardware restriction and searching difficulty for NAS problems. NAS or even AutoML can be widely applied to various situations.
